Towards Revealing the Mystery behind Chain of Thought: A Theoretical Perspective

Recent studies have discovered that Chain-of-Thought prompting (CoT) can dramatically improve the performance of Large Language Models (LLMs), particularly when dealing with complex tasks involving mathematics or reasoning. Despite the enormous empirical success, the underlying mechanisms behind CoT and how it unlocks the potential of LLMs remain elusive. In this paper, we take a first step towards theoretically answering these questions. Specifically, we examine the expressivity of LLMs with CoT in solving fundamental mathematical and decision-making problems. By using circuit complexity theory, we first give impossibility results showing that bounded-depth Transformers are unable to directly produce correct answers for basic arithmetic/equation tasks unless the model size grows super-polynomially with respect to the input length. In contrast, we then prove by construction that autoregressive Transformers of constant size suffice to solve both tasks by generating CoT derivations using a commonly used math language format. Moreover, we show LLMs with CoT can handle a general class of decision-making problems known as Dynamic Programming, thus justifying its power in tackling complex real-world tasks. Finally, an extensive set of experiments show that, while Transformers always fail to directly predict the answers, they can consistently learn to generate correct solutions step-by-step given sufficient CoT demonstrations.

==> Old_Files/proof_poly.tex <==
\section{Polynomial Simplification}

In this section, we will prove that the autoregressive transformer can solve the arithmetic formula using the chain of thought we demonstrated earlier, whereas the autoregressive transformer without the chain of thought cannot solve the arithmetic formula. 

First, we will prove the theorem, demonstrating that the transformer can calculate the formula with the previous chain of thought. 


\begin{theorem}

    Given any $L$ and any prime $p$, there exists an autoregressive transformer with embeddings of size $O(p)$, hidden dimension of $O(poly(p))$, $3$ layers, and $5$ attention head in each layer that can output the CoT for all arithmetic formulas modulo $p$ of length at most $L$. Moreover, the weight norm of the transformer is bounded by $O(poly(L))$. 

\end{theorem}

First, we give an overview of the proof.  The intuition behind the construction is that when the transformer output part of the expression, it can determine whether this location can be calculated by checking several tokens behind it. Based on the key observation, we can construct our four-layer transformer. The first layer counts the number of equal signs in the previous tokens and copies the position index of the last equal sign. The second layer determines whether to perform a calculation by examining the current token and the five tokens immediately behind it. The third layer and the fourth layer generate a sequence of tokens using the outcomes of the previous layer. The transformer can be trained using a maximum likelihood objective function. The authors demonstrate the effectiveness of their method on two tasks: generating mathematical expressions and generating computer programs.


\begin{proof}

    \item
    \paragraph{Token Embeddings}
    Assuming that we have a sequence of tokens $t_1, \ldots, t_n$ and we want to generate the next token $t_{n+1}$, we can embed the token $t_i$ using the format $v_{i,0}=[e_i, i, 1]$, where $e_i$ is a one-hot vector that represents the $i$-th token in the vocabulary. The position embedding $i$ represents the position of the token in the sequence, and the constant embedding $1$ is used as a bias term.
    
    \paragraph{Layer 1}
    The first layer of the autoregressive transformer uses two attention heads to perform the following tasks:
    \begin{enumerate}
        \item Count the number of equal signs in the previous tokens, denoted as $n_{eq}$.
        \item Copy the position index of the last equal sign, denoted as $p_{eq}$.
    \end{enumerate}
    According to the previous lemma, the first attention head of the autoregressive transformer counts the number of equal signs in the previous tokens, denoted as $n_{eq}$. The second attention head performs the COPY operation to copy the position index of the last equal sign, denoted as $p_{eq}$. The output of the attention layer is then given by $[e_i, i, 1, n_{eq}/i, p_{eq}]$. We can use an MLP to multiply $n_{eq}/i$ and $i$ to obtain $n_{eq}$ and compute the distance between the last equal sign and the current position $d_{eq}$, by subtracting $p_{eq}$ from $i$ and adding $1$. These operations can be simply done according to the previous lemmas. Therefore, the final output of the first layer is $v_{i,1}=[e_i, i, n_{eq,i}, d_{eq,i},n_{eq,i}^2, d_{eq,i}^2 ,1]$.

    \paragraph{Layer 2}
    The intuition behind the second layer of the autoregressive transformer is that it can determine whether to perform a calculation by examining the current token and the five tokens immediately behind it. This observation is crucial for constructing the transformer and can be easily verified by enumerating all possible cases. Therefore this layer utilizes five attention heads to perform the following tasks:
    \begin{enumerate}
        \item Copy the embedding $e_j$ located at position $j$ such that $n_{eq,j}=n_{eq,i}-1$ and $d_{eq,j}=d_{eq,i}+k$ for $k=1,2,3,4,5$.
        \item Check if the copied expression can be evaluated, if it can be calculated, compute its outcome and maintain the token otherwise, and determine how many tokens the expression will decrease by.
    \end{enumerate}
    We can utilize the COPY operation five times in parallel for the attention layer. For each $k$, we can construct the matrices $K$ and $Q$ of the COPY operation such that $Kv_{i,1}=[n^2_{eq,i}-2n_{eq,i}+1,1,n_{eq,i}-1,d^2_{eq,i}-2kn_{eq,i}+k^2,1,d_{eq,i}-k]$ and $Qv_{i,1}=[1,n^2_{eq,i},-2n_{eq,i},1,d^2_{eq,i},-2d_{eq,i}]$. These matrices satisfy that $Kv_{i,1}\cdot Qv_{j,1}=0$ only when $n_{eq,j}=n_{eq,i}-1$ and $d_{eq,j}=d_{eq,i}+k$, and $Kv_{i,1}\cdot Qv_{j,1}\geq 1$ otherwise. So the output of the attention layer is $[e_i,e_{j_1},e_{j_2},e_{j_3},e_{j_4},e_{j_5} i, n_{eq, i}, d_{eq, i},n_{eq, i}^2, d_{eq,i}^2,1]$, where $e_{j_k}$ is the embedding we copied by the five attention heads. We can use an MLP in the second layer to perform the second task. As all the embeddings are one-hot vectors, we can use a fixed number of hidden dimensions to determine whether the expression can be calculated or not. For instance, we can enumerate all cases of the types of the six tokens in the hidden layer. If the expression can be calculated, we can use a larger number of hidden dimensions, typically $O(p^2)$, to memorize the computation table and compute the outcome. Lastly, a fixed number of hidden dimensions can be used to determine the length of the expression that will be decreased. Therefore, the output of the second layer is represented by $v_{i,2}=[e_{outcome,i}, e_{j_1}, tag_i, d_{eq,i},n_{eq,i}, num_i]$. Here, $e_{outcome,i}$ is the one-hot embedding of the outcome, $tag_i$ records whether the copied expression can be calculated, and $num_i$ records the length of the expression that will be decreased.
    
    \paragraph{Layer 3}
    The third layer of the autoregressive transformer utilizes two attention heads to perform the following tasks: 
    \begin{enumerate}
        \item Copy the embedding $num_j$ located at position $j$ such that $n_{eq,j}=n_{eq,i}$.
        \item MEAN over the $tag_i$ of the embedding $v_{j,2}$ such that $n_{eq,j}=n_{eq,i}$.
        \item Filter the outcome. I.e. if $tag_i=1$, then maintain $e_{outcome,i}$ and set $e_{j_1}=0$ and if $tag_i=0$ then maintain $e_{j_1}$ and set $e_{outcome,i}=0$.
    \end{enumerate}
    Similar to the construction of the second layer, we can construct the matrices $K$ and $Q$ of the COPY operation and the MEAN operation such that $Kv_{i,1}=[n^2_{eq, i},n_{eq, i},1]$ and $Qv_{i,1}=[1,n^2_{eq, i},-2n_{eq, i}]$. These matrices satisfy that $Kv_{i,1}\cdot Qv_{j,1}=(n_{eq,i}-n_{eq,j})^2$ only when $n_{eq,j}=n_{eq,i}-1$ and $d_{eq,j}=d_{eq,i}+k$, and $Kv_{i,1}\cdot Qv_{j,1}\geq 1$ otherwise. So the output of the attention layer is $[e_{outcome,i},e_{j_1}, tag_i, d_{eq,i},n_{eq,i}, num_i,tag_{i}^\prime/d_{eq,i},num_i^\prime]$, where $tag_{i}^\prime$ record is this expression has been calculated and $num^i\prime$ record the length decreased by. So passing the embedding through the MLP, we can obtain the embedding $v_{i,3}=[e_{outcome,i},e_{j_1}, tag_i, d_{eq,i},n_{eq,i}, num_i,tag_{i}^\prime,num_i^\prime]$

    

    \paragraph{Layer 4}
    The final layer of the autoregressive transformer uses one attention head to copy the corresponding position and filter to get the output. Similar to the second layer, we can copy the embedding $e_j$ located at position $j$ such that $n_{eq,j}=n_{eq,i}-1$ and $d_{eq,j}=d_{eq,i}+num_i^\prime$. Therefore the output of the attention layer is $[e_{outcome,i},e_{j_1},e_{j} tag_i, d_{eq,i},n_{eq,i}, num_i,tag_{i}^\prime,num_i^\prime]$, where $e_j$ is the token we can copied. Then we pass the embeddings through the MLP to filter and obtain the output. If $tag_i^\prime=1$, then maintain $e_{j}$ and set $e_{j_1}=0,e_{outcome,i}=0$ and if $tag_i=0$ then maintain $e_{j_1}$ and $e_{outcome,i}$ and set $e_{j}=0$. So the output of the MLP is $[e_{j_1},e_{j},e_{outcome,i}]$ and only one of them is a one-hot vector and others are zero vectors.

    Finally, we pass it through a softmax layer to get the next token $t_{n+1}$.

    Note that, we can tolerate $O(1)$(at most $0.5$) error of the output of the fourth layer and the $L_\infty$ norm embedding of the inner layer is bounded by $L^2$. So according to the previous lemma, the weight norm of the transformer constructed in this proof is bounded by $O(poly(L))$

\end{proof}

We will now prove that calculating an arithmetic formula without the chain of thought is extremely difficult for the autoregressive transformer. To do this, we will assume that $TC^0$ is not equal to $NC^1$-uniform $NC^1$. Note that this is a significant open question in computation theory, as it is still unclear whether $TC^0$ is equal to $NC^1$-uniform $NC^1$. However, for the purpose of this proof, we will make this assumption. According to the previous work, calculating the value of a boolean formula is complete for $NC^1$-uniform $NC^1$. Based on the assumption and the theorem, we only need to prove that calculating the arithmetical formula is also complete for $NC^1$-uniform $NC^1$.

\begin{theorem}

    For any autoregressive transformer with constant layers, there exists a $L$, it can't calculate the outcome of an arithmetic formula modulo $p$ of length  $L$ property. 
    
\end{theorem}

\begin{proof}

    
With the assumption that $TC^0 \neq NC^1$-uniform $NC^1$ and the previous theorem, we can now focus on proposing a reduction from the problem of calculating the value of a boolean formula to the problem of calculating an arithmetic formula modulo $p$. 

For any boolean formula, it must have one of the following forms:
\begin{enumerate}
    \item $x\land y$
    \item $x\lor y$
    \item $\neg x$
\end{enumerate}
We have $x\land y=x\cdot y$, $x\lor y=1-(1-x)\cdot (1-y)$ and $\neg x= 1-x$, for all $x,y\in \{0,1\}$. So we can simply convert the boolean formula to an arithmetical formula and the values of the two formulas are exactly the same. We can see that the reduction can be done by a constant depth circuit. So the problem of calculating an arithmetic formula modulo $p$ is also complete for $NC^1$-uniform $NC^1$.
\end{proof}



